Functions with constant Laplacian satisfying Robin boundary conditions on an ellipse

(Version 3) We study the problem of finding functions, defined within and on an ellipse, whose Laplacian is -1 and which satisfy a homogeneous Robin boundary condition on the ellipse. The parameter in the Robin condition is denoted by beta. The general solution and various asymptotic approximations are obtained. The integral of the solution over the ellipse, denoted by Q, is a quantity of interest in some physical applications. The dependence of Q on beta and the ellipse geometry is found. Several methods are used.

==> keadyEllRAppCode.tex <==


\section{Code producing the Figure}

\verbatiminput{/Users/grantkeady/Documents/MIcrochannels/Ellipse/Mathca/rApproxPlotmma.txt}


